Labeling Explicit Discourse Relations using Pre-trained Language Models

Labeling explicit discourse relations is one of the most challenging sub-tasks of the shallow discourse parsing where the goal is to identify the discourse connectives and the boundaries of their arguments. The state-of-the-art models achieve slightly above 45% of F-score by using hand-crafted features. The current paper investigates the efficacy of the pre-trained language models in this task. We find that the pre-trained language models, when finetuned, are powerful enough to replace the linguistic features. We evaluate our model on PDTB 2.0 and report the state-of-the-art results in the extraction of the full relation. This is the first time when a model outperforms the knowledge intensive models without employing any linguistic features.

==> README <==
academicons -- high quality icons of online academic profiles

The "academicons" package provides access in (La)TeX to 76 high quality icons
of online academic profiles included in the free "Academicons" font. This
package requires either the Xe(La)TeX or Lua(La)TeX engine to load the
"Academicons" font from the system, which requires installing the bundled
"academicons.ttf" font file. As new releases come out, it is recommended to
install the bundled font version as there may be differences between the package
and previous font versions or newest font versions not yet contemplated in the
package.

The "Academicons" font was designed by James Walsh and released (see
http://jpswalsh.github.io/academicons/) under the open SIL Open Font License
(available at http://scripts.sil.org/OFL). This package is a redistribution of
the free "Academicons" font with specific bindings for (La)TeX. It is inspired
and based on the "fontawesome" package (available at
http://www.ctan.org/pkg/fontawesome).

The academicons package provides the generic "\aiicon" command to access icons,
which takes as mandatory argument the name of the desired icon. It also
provides individual direct commands for each specific icon. The full list of
icons and their respective names and direct commands can be found in the
manual. For example, "\aiicon{googlescholar}" yields the same result as
"\aiGoogleScholar".

academicons (La)TeX package
https://www.ctan.org/pkg/academicons
Version: 1.8.6-2
Author: Diogo A. B. Fernandes, diogoabfernandes at gmail.com
License: LaTeX Project Public License, version 1.3c

Academicons font
Author: James Walsh
Licence: SIL Open Font License, version 1.1

